Dual Thinking and Logical Processing -- Are Multi-modal Large Language Models Closing the Gap with Human Vision ?

The dual thinking framework considers fast, intuitive, and slower logical processing. The perception of dual thinking in vision requires images where inferences from intuitive and logical processing differ, and the latter is under-explored in current studies. We introduce a novel adversarial dataset to provide evidence for the dual thinking framework in human vision, which also facilitates the study of the qualitative behavior of deep learning models. Our psychophysical studies show the presence of multiple inferences in rapid succession, and analysis of errors shows that the early stopping of visual processing can result in missing relevant information. MLLMs (Multi-modal Large Language Models) and VLMs (Vision Language Models) have made significant progress in correcting errors in intuitive processing in human vision and showed enhanced performance on images requiring logical processing. However, their improvements in logical processing have not kept pace with their advancements in intuitive processing. In contrast, segmentation models exhibit errors similar to those seen in intuitive human processing and lack understanding of sub-structures, as indicated by errors related to sub-components in identified instances. As AI (Artificial Intelligence)-based systems find increasing applications in safety-critical domains like autonomous driving, the integration of logical processing capabilities becomes essential. This not only enhances performance but also addresses the limitations of scaling-based approaches while ensuring robustness and reliability in real-world environments.

==> tables/gestalt_table.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
Model & FG \dag & Proximity & Similarity & Continuity & Amodal & Global Mix & Size Diff & Count Diff & Camo \ddag \\
\midrule
DetectoRS-R50 & 0.38 & 0.25 & 0.27 & 0.22 & 0.46 & 0.17 & 0.17 & 0.05 & 0.32 \\
DetectoRS-R101 & 0.38 & 0.24 & 0.27 & 0.23 & 0.48 & 0.16 & 0.09 & 0.03 & 0.3 \\
M-RCNN-R50 & 0.3 & 0.17 & 0.2 & 0.2 & 0.48 & 0.08 & 0.07 & 0.05 & 0.14 \\
M-RCNN-R101 & 0.34 & 0.2 & 0.24 & 0.22 & 0.48 & 0.1 & 0.13 & 0.05 & 0.22 \\
M-RCNN-X101 & 0.35 & 0.2 & 0.25 & 0.21 & 0.62 & 0.11 & 0.11 & 0.03 & 0.24 \\
YOLACT-R50 & 0.26 & 0.13 & 0.14 & 0.13 & 0.23 & 0.04 & 0.06 & 0.03 & 0.15 \\
YOLACT-R101 & 0.24 & 0.13 & 0.14 & 0.13 & 0.25 & 0.02 & 0.07 & 0.03 & 0.1 \\
Swin-T & 0.38 & 0.25 & 0.28 & 0.26 & 0.63 & 0.22 & 0.17 & 0.05 & 0.3 \\
Swin-S & 0.4 & 0.28 & 0.3 & 0.27 & 0.66 & 0.29 & 0.13 & 0.1 & 0.36 \\
Instaboost-R50 & 0.32 & 0.18 & 0.21 & 0.21 & 0.48 & 0.08 & 0.09 & 0.05 & 0.17 \\
Instaboost-R101 & 0.37 & 0.22 & 0.26 & 0.22 & 0.52 & 0.08 & 0.09 & 0.05 & 0.28 \\
Instaboost-X101 & 0.36 & 0.22 & 0.25 & 0.22 & 0.58 & 0.14 & 0.11 & 0.03 & 0.25 \\
GROIE-R50 & 0.35 & 0.21 & 0.25 & 0.23 & 0.54 & 0.1 & 0.11 & 0.05 & 0.23 \\
GROIE-R101 & 0.38 & 0.22 & 0.26 & 0.23 & 0.58 & 0.07 & 0.15 & 0.05 & 0.25 \\
GPT-4o & \textbf{0.88} & \textbf{0.77} & \textbf{0.75} & \textbf{0.68} & 0.63 & \textbf{0.9} & 0.37 & 0.64 & \textbf{0.93} \\
GPT-4o-mini & 0.73 & 0.71 & 0.69 & \textbf{0.68} & \textbf{0.7} & 0.76 & \textbf{0.61} & \textbf{0.82} & 0.74 \\
Llama-3.2-11B & 0.71 & 0.67 & 0.64 & 0.6 & 0.48 & 0.84 & 0.5 & 0.69 & 0.79 \\
\bottomrule
{\raggedright \dag Figure Ground.}\\ 
{\ddag Camouflage}
\end{tabular}


==> tables/gestalt_table_both.tex <==
\begin{tabular}{llrrrrrrrrr}
\toprule
Property & Model & FG \dag & Proximity & Similarity & Continuity & Amodal & Global Mix & Size Diff & Count Diff & Camo \ddag \\
\midrule
 & DetectoRS-R50 & 0.38 & 0.25 & 0.27 & 0.22 & 0.46 & 0.17 & 0.17 & 0.05 & 0.32 \\
 & DetectoRS-R101 & 0.38 & 0.24 & 0.27 & 0.23 & 0.48 & 0.16 & 0.09 & 0.03 & 0.3 \\
 & M-RCNN-R50 & 0.3 & 0.17 & 0.2 & 0.2 & 0.48 & 0.08 & 0.07 & 0.05 & 0.14 \\
 & M-RCNN-R101 & 0.34 & 0.2 & 0.24 & 0.22 & 0.48 & 0.1 & 0.13 & 0.05 & 0.22 \\
Correct & M-RCNN-X101 & 0.35 & 0.2 & 0.25 & 0.21 & 0.62 & 0.11 & 0.11 & 0.03 & 0.24 \\
 & YOLACT-R50 & 0.26 & 0.13 & 0.14 & 0.13 & 0.23 & 0.04 & 0.06 & 0.03 & 0.15 \\
 & YOLACT-R101 & 0.24 & 0.13 & 0.14 & 0.13 & 0.25 & 0.02 & 0.07 & 0.03 & 0.1 \\
 & Swin-T & 0.38 & 0.25 & 0.28 & 0.26 & 0.63 & 0.22 & 0.17 & 0.05 & 0.3 \\
 & Swin-S & 0.4 & 0.28 & 0.3 & 0.27 & 0.66 & 0.29 & 0.13 & 0.1 & 0.36 \\
 & Instaboost-R50 & 0.32 & 0.18 & 0.21 & 0.21 & 0.48 & 0.08 & 0.09 & 0.05 & 0.17 \\
 & Instaboost-R101 & 0.37 & 0.22 & 0.26 & 0.22 & 0.52 & 0.08 & 0.09 & 0.05 & 0.28 \\
 & Instaboost-X101 & 0.36 & 0.22 & 0.25 & 0.22 & 0.58 & 0.14 & 0.11 & 0.03 & 0.25 \\
 & GROIE-R50 & 0.35 & 0.21 & 0.25 & 0.23 & 0.54 & 0.1 & 0.11 & 0.05 & 0.23 \\
 & GROIE-R101 & 0.38 & 0.22 & 0.26 & 0.23 & 0.58 & 0.07 & 0.15 & 0.05 & 0.25 \\
 & GPT-4o & \textbf{0.88} & \textbf{0.77} & \textbf{0.75} & \textbf{0.68} & 0.63 & \textbf{0.9} & 0.37 & 0.64 & \textbf{0.93} \\
 & GPT-4o-mini & 0.73 & 0.71 & 0.69 & \textbf{0.68} & \textbf{0.7} & 0.76 & \textbf{0.61} & \textbf{0.82} & 0.74 \\
 & Llama-3.2-11B & 0.71 & 0.67 & 0.64 & 0.6 & 0.48 & 0.84 & 0.5 & 0.69 & 0.79 \\
\midrule
\midrule
 & DetectoRS-R50 & 0.45 & 0.49 & 0.49 & 0.48 & 0.25 & 0.31 & 0.72 & \textbf{0.72} & 0.56 \\
 & DetectoRS-R101 & 0.48 & \textbf{0.52} & \textbf{0.52} & \textbf{0.5} & 0.27 & 0.33 & \textbf{0.81} & 0.62 & 0.61 \\
 & M-RCNN-R50 & 0.47 & 0.47 & 0.46 & 0.39 & 0.18 & 0.23 & 0.59 & 0.54 & 0.71 \\
 & M-RCNN-R101 & 0.45 & 0.47 & 0.45 & 0.43 & 0.21 & 0.22 & 0.61 & 0.51 & 0.66 \\
Human & M-RCNN-X101 & 0.45 & 0.49 & 0.47 & 0.44 & 0.18 & 0.27 & 0.65 & 0.62 & 0.63 \\
 & YOLACT-R50 & 0.5 & 0.48 & 0.47 & 0.39 & 0.14 & 0.37 & 0.59 & 0.46 & 0.78 \\
 & YOLACT-R101 & \textbf{0.54} & 0.5 & 0.49 & 0.41 & 0.13 & 0.34 & 0.61 & 0.49 & \textbf{0.82} \\
 & Swin-T & 0.43 & 0.45 & 0.46 & 0.42 & 0.24 & 0.14 & 0.65 & 0.59 & 0.57 \\
 & Swin-S & 0.41 & 0.45 & 0.46 & 0.45 & 0.27 & 0.16 & 0.74 & 0.62 & 0.51 \\
 & Instaboost-R50 & 0.48 & 0.49 & 0.48 & 0.42 & 0.15 & 0.29 & 0.56 & 0.56 & 0.71 \\
 & Instaboost-R101 & 0.44 & 0.47 & 0.45 & 0.42 & 0.18 & 0.27 & 0.65 & 0.62 & 0.6 \\
 & Instaboost-X101 & 0.47 & 0.5 & 0.48 & 0.45 & 0.21 & 0.23 & 0.65 & 0.56 & 0.65 \\
 & GROIE-R50 & 0.46 & 0.48 & 0.47 & 0.42 & 0.2 & 0.29 & 0.63 & 0.59 & 0.64 \\
 & GROIE-R101 & 0.46 & 0.49 & 0.48 & 0.46 & 0.24 & \textbf{0.39} & 0.63 & 0.59 & 0.63 \\
 & GPT-4o & 0.11 & 0.22 & 0.25 & 0.31 & 0.37 & 0.1 & 0.61 & 0.36 & 0.05 \\
 & GPT-4o-mini & 0.26 & 0.28 & 0.3 & 0.32 & 0.28 & 0.24 & 0.39 & 0.18 & 0.25 \\
 & Llama-3.2-11B & 0.29 & 0.32 & 0.35 & 0.39 & \textbf{0.51} & 0.16 & 0.48 & 0.28 & 0.21 \\
\bottomrule
{\raggedright \dag Figure Ground.}\\ 
{\ddag Camouflage}
\end{tabular}


==> tables/gestalt_table_human.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
Model & FG \dag & Proximity & Similarity & Continuity & Amodal & Global Mix & Size Diff & Count Diff & Camo \ddag \\
\midrule
DetectoRS-R50 & 0.45 & 0.49 & 0.49 & 0.48 & 0.25 & 0.31 & 0.72 & \textbf{0.72} & 0.56 \\
DetectoRS-R101 & 0.48 & \textbf{0.52} & \textbf{0.52} & \textbf{0.5} & 0.27 & 0.33 & \textbf{0.81} & 0.62 & 0.61 \\
M-RCNN-R50 & 0.47 & 0.47 & 0.46 & 0.39 & 0.18 & 0.23 & 0.59 & 0.54 & 0.71 \\
M-RCNN-R101 & 0.45 & 0.47 & 0.45 & 0.43 & 0.21 & 0.22 & 0.61 & 0.51 & 0.66 \\
M-RCNN-X101 & 0.45 & 0.49 & 0.47 & 0.44 & 0.18 & 0.27 & 0.65 & 0.62 & 0.63 \\
YOLACT-R50 & 0.5 & 0.48 & 0.47 & 0.39 & 0.14 & 0.37 & 0.59 & 0.46 & 0.78 \\
YOLACT-R101 & \textbf{0.54} & 0.5 & 0.49 & 0.41 & 0.13 & 0.34 & 0.61 & 0.49 & \textbf{0.82} \\
Swin-T & 0.43 & 0.45 & 0.46 & 0.42 & 0.24 & 0.14 & 0.65 & 0.59 & 0.57 \\
Swin-S & 0.41 & 0.45 & 0.46 & 0.45 & 0.27 & 0.16 & 0.74 & 0.62 & 0.51 \\
Instaboost-R50 & 0.48 & 0.49 & 0.48 & 0.42 & 0.15 & 0.29 & 0.56 & 0.56 & 0.71 \\
Instaboost-R101 & 0.44 & 0.47 & 0.45 & 0.42 & 0.18 & 0.27 & 0.65 & 0.62 & 0.6 \\
Instaboost-X101 & 0.47 & 0.5 & 0.48 & 0.45 & 0.21 & 0.23 & 0.65 & 0.56 & 0.65 \\
GROIE-R50 & 0.46 & 0.48 & 0.47 & 0.42 & 0.2 & 0.29 & 0.63 & 0.59 & 0.64 \\
GROIE-R101 & 0.46 & 0.49 & 0.48 & 0.46 & 0.24 & \textbf{0.39} & 0.63 & 0.59 & 0.63 \\
GPT-4o & 0.11 & 0.22 & 0.25 & 0.31 & 0.37 & 0.1 & 0.61 & 0.36 & 0.05 \\
GPT-4o-mini & 0.26 & 0.28 & 0.3 & 0.32 & 0.28 & 0.24 & 0.39 & 0.18 & 0.25 \\
Llama-3.2-11B & 0.29 & 0.32 & 0.35 & 0.39 & \textbf{0.51} & 0.16 & 0.48 & 0.28 & 0.21 \\
\bottomrule
{\raggedright \dag Figure Ground.}\\ 
{\ddag Camouflage}
\end{tabular}

